Self-assessment, Exhibition, and Recognition: a Review of Personality in Large Language Models

As large language models (LLMs) appear to behave increasingly human-like in text-based interactions, more and more researchers become interested in investigating personality in LLMs. However, the diversity of psychological personality research and the rapid development of LLMs have led to a broad yet fragmented landscape of studies in this interdisciplinary field. Extensive studies across different research focuses, different personality psychometrics, and different LLMs make it challenging to have a holistic overview and further pose difficulties in applying findings to real-world applications. In this paper, we present a comprehensive review by categorizing current studies into three research problems: self-assessment, exhibition, and recognition, based on the intrinsic characteristics and external manifestations of personality in LLMs. For each problem, we provide a thorough analysis and conduct in-depth comparisons of their corresponding solutions. Besides, we summarize research findings and open challenges from current studies and further discuss their underlying causes. We also collect extensive publicly available resources to facilitate interested researchers and developers. Lastly, we discuss the potential future research directions and application scenarios. Our paper is the first comprehensive survey of up-to-date literature on personality in LLMs. By presenting a clear taxonomy, in-depth analysis, promising future directions, and extensive resource collections, we aim to provide a better understanding and facilitate further advancements in this emerging field.

==> Evaluating_Personality.tex <==
\section{LLM's Personality Self-assessment}
\label{LLM's Personality Self-assessment}

\textit{Does a LLM possess a stable personality trait?} This question arises from the highly coherent and human-like conversational experience provided by LLMs during interactions, which drives researchers to investigate whether LLMs have acquired intrinsic personality traits in pre-training. Some studies \cite{huang2023chatgptMBTI, pan2023llms} suggest that ChatGPT approximates a stable ENFJ personality type in the MBTI model, while others indicate that LLMs do not consistently maintain a personality trait in assessments \cite{pellert2022ai,miotto2022gpt}. The discrepancy may stem from variations in methodology or the inherent adaptability of LLMs to different conversational contexts. Understanding LLMs' personalities not only helps enrich the user experience by fostering engaging and empathetic interactions but also plays a crucial role in uncovering latent biases, mitigating the biases, and thereby enhancing the fairness and accuracy of LLMs \cite{karra2022estimating}. 

\subsection{Problem Definition}
We first define the LLM's Personality Self-assessment problem as: \textbf{How to systematically measure the personality traits exhibited in text responses from LLMs through psychometric methods?} The psychometric methods means can be both direct psychometric questionnaires and text analysis based on psychology domain knowledge. This problem is based on an important assumption: (1) Due to LLMs being trained on vast corpora of human-written text that routinely contains statements related to human values, attitudes, beliefs, and personality traits, such models will inadvertently but inevitably acquire a set of psychological characteristics during the training process \cite{pellert2022ai}, 

\subsection{How do people assess the personalities of LLMs?}

When assessing human personality, researchers commonly employ personality questionnaires and self-report essays. Similarly, existing studies also conduct several main approaches to investigate the intrinsic personality traits of LLMs:  (1) prompting LLMs with Likert scale personality questionnaires, and (2) analyzing the textual responses of LLMs. We will introduce these methods in the following content.

\subsubsection{Likert scale questionnaires}

Likert scale-based personality questionnaires (\textit{e.g.}, Table \ref{BFI_example}) consist of a series of multiple-choice questions that map respondents' choices to various scores, which are then aggregated to yield a final result. These instruments are frequently utilized in the social sciences to assess the personality traits of humans. 

Researchers (\textit{e.g.}, \citet{caron2022identifying,jiang2023evaluating}) have endeavored to employ such questionnaires for LLMs by inputting the questionnaire items and constraining the response format to obtain the personality traits exhibited by LLMs. 
These studies assume that these questionnaires for personality assessment for LLMs methods designed for humans can also measure personality in LLMs \cite{song2023large}.


\begin{table}[t]
    \centering
    \linespread{1}
    \renewcommand{\arraystretch}{1.3}
    \begin{tabular}{p{7cm}}
 	\toprule
 	\textit{I see myself as someone who is helpful and unselfish with others.}   \\
	\hline
	\textit{1 = Disagree strongly} \\
	\textit{2 = Disagree a little} \\
	\textit{3 = Neither agree nor disagree} \\
	\textit{4 = Agree a little} \\
	\textit{5 = Agree strongly} \\
	\hline
	\textit{Please write a number to indicate the extent to which you agree or disagree with that statement.}\\
	\bottomrule
    \end{tabular}
    \caption{The 7-th question in the BFI \cite{john1999big}.}
    \label{BFI_example}
\end{table}

One common approach to utilizing questionnaires to assess the personality of LLMs is to modify the questionnaire items with prompting engineering to make them suitable for the input of LLMs. Earlier work \cite{caron2022identifying} first explored assessing the big-five personality traits of BERT and GPT-2 by a personality questionnaire \cite{goldberg2006administering}. They modify the questionnaire by incorporating blanks within the item questions. Then, the models are expected to select the options that best fit the blanks. 
\cite{miotto2022gpt} rephrases the items in the HEXACO questionnaire into the third person plural as the prompts and asks GPT-3 to answer the extent of how much the descriptions are similar to itself. The overall scores obtained from GPT-3 are then compared with the HEXACO scores of human participants. 
\cite{li2023does} adds an instruction containing all available options (\textit{e.g., Do you agree, slightly agree, disagree,...,? }) beside each original question in the personality inventories as the input for LLMs. 
Furthermore, some studies \cite{jiang2023evaluating,lacava2024open,sorokovikova2024llms,huang2023chatgpt} added instructive task descriptions and constraints such as \textit{You will be provided a question ... to test your personality} and \textit{To answer this question using only one number: write 1 if you disagree strongly...} to constraint the output format of LLMs.

Since most LLMs are trained with Supervised Fine-Tuning (SFT) to have conversation and question-answering capabilities, their responses tend to be natural sentences rather than precise questionnaire answer options. Therefore, many studies also attempt to extract answer options from the responses to obtain assessment results. \cite{safdari2023personality}  instruct LLMs to rate items from each personality questionnaire on a standardized response scale. Then, they simulated the LLM’s chosen response to each item by ranking the conditional log probabilities of the response scale options. Similarly, the authors of \cite{pan2023llms} prompt the LLM with multi-choice questions within personality inventories. Subsequently, they analyze the probability values of the last token in the text response generated by the LLM and select the options with the highest probability as the model's answer.

\subsubsection{Text response analysis}

Despite most existing studies utilizing questionnaires to assess the personalities of LLMs, some researchers \cite{dorner2023personality, huang2023revisiting} also question the suitability of directly employing psychological scales, initially devised for humans, on LLMs for personality assessment. Therefore, there are also studies that conduct text analysis on the responses of LLMs to questionnaires or context descriptions to determine their personalities. 

\cite{karra2022estimating} classifies the text responses of LLMs to a personality questionnaire into the big five personality traits using a Zero-shot classifier. Similarly, \cite{pellert2022ai} prompted the questions from personality inventories recorded the language models' responses, and conducted zero-shot classification to obtain their personality scores. While \cite{hilliard2024eliciting} measures the Big Five personality traits of LLMs by further classify their responses to prompts derived from standard interview questions with fine-tuned text classifiers. Besides end-to-end text classifiers, Linguistic Inquiry and Word Count (LIWC, \citet{pennebaker2001linguistic}), a text analysis tool for personality recognition is also adopted in existing studies \cite{frisch2024llm,gu2023effectiveness,jiang2023personallm} for personality assessment of LLMs. It's worth mentioning that \cite{jiang2023evaluating} also conducts the vignette test \cite{kwantes2016assessing} to assess the personality exhibited by LLMs. They prompt LLMs with the context that describes a real-world scenario, followed by an open question and instructions for a short essay. Then, human participants were recruited to assess the generated responses of LLMs in personality reflection.


\subsection{What are the assessment results?}

Based on the various assessment methods introduced above, researchers have obtained the results of personality of LLMs. In general,  although the results are similar in some aspects, they are different as a whole. These differences depend on a variety of factors: measurement approaches, model versions, hyperparameters, and so on.

Categorical results: 

\begin{table}[t]
    \centering
    \linespread{1.2}
    \small
    \begin{tabular}{lcc}
 	\hline
	\textbf{LLMs}  & \textbf{Results} & \textbf{Source} \\
\hline
ChatGPT &  ENTJ &  \cite{pan2023llms} \\
ChatGPT &  ENFJ &  \cite{huang2023chatgptMBTI} \\
GPT-4 &  INTJ & \cite{pan2023llms} \\
GPT-4 &  ENFJ & \cite{huang2023chatgptMBTI} \\
Llama-7b  & ENFP & \cite{pan2023llms} \\
Llama-2 (7b,13b) & ENFJ & \cite{pan2023llms} \\
\hline
    \end{tabular}
    \caption{Personality Traits.}
    \label{result_overall}
\end{table}

Numeric Results: Big-five and Dark Triad (How are they compared with human scores?)

\cite{karra2022estimating}
\cite{bodroza2023personality}
\cite{miotto2022gpt}
\cite{li2023does}
\cite{huang2023revisiting} In the OCEAN dimensions, gpt-3.5-turbo records standard deviations of 0.3, 0.3, 0.4, 0.3, and 0.4, respectively, while the crowd data show a higher variability with 0.7, 0.7, 0.9, 0.7, and 0.8.
\cite{huang2023chatgpt}
\cite{huang2023chatgpt}
\cite{romero2023gpt}
\cite{hilliard2024eliciting}
\cite{dorner2023personality}
\cite{sorokovikova2024llms}
\cite{frisch2024llm}
\cite{jiang2023evaluating}


\textcolor{red}{why the same model evolve?} It is worth noting \cite{huang2023revisiting} long-term observation...\\

\noindent
\textbf{Findings 1}: Previous research on emergence in large language models shows these display apparent human-like abilities and psychological latent traits. However, results are partly contradicting in expression and magnitude of these latent traits, yet agree on the worrisome tendencies to score high on the Dark Triad of narcissism, psychopathy, and Machiavellianism, which, together with a track record of derailments, demands more rigorous research on the safety of these models. 


\subsection{Are the assessments robust?}

Due to the diversity of the assessment results, researchers investigate the robustness of the assessments from different aspects. Although multiple terms are used and interpreted, such as reliability \cite{huang2023revisiting}, stability \cite{shu2024dont}, self-consistency \cite{pellert2022ai}, and validity \cite{romero2023gpt}, we summarize these terms mainly are from two perspectives:
\textbf{Reliability}, which refers to measurement precision and can be approximated by the consistency of answers and the stability of test results over multiple repetitions; and \textbf{Validity}, which refers to the extent to which a test measures what it claims to measure, in other words, whether the personality assessment approaches used are indeed applicable to measuring the personalities of LLMs \cite{dorner2023personality}. The former explores the results from the perspective of the LLMs, while the latter investigates from the perspective of the assessment approaches.

\subsubsection{Reliability}
Several studies have reported achieving high reliability in the personality assessments of LLMs. \cite{huang2023revisiting} conducted a comprehensive analysis of responses across 2,500 experimental conditions, demonstrating that GPT-3.5-turbo exhibits consistent behavior in responses to the Big Five Inventory. \cite{jiang2023evaluating} further bolstered this notion, performing multiple analyses to illustrate that GPT-3.5 can manifest consistent personality tendencies throughout numerous evaluations. In a related study, \cite{huang2023mbti} showcased that ChatGPT consistently exhibits the ENFJ personality type across diverse languages, prompts, question orders, and rephrased inquiries in assessments.

However, not all findings are in agreement. \cite{li2023does}, while asserting that GPT-3 displays relatively consistent personality traits, also identified instances of conflicting answers and discrepancies in the responses generated by LLMs attributable to variations in the order of options within prompts. \cite{gupta2024selfassessment} discovered that the test scores of ChatGPT and Llama-2 are not consistently robust across equivalent prompts and differing option presentations. Additionally, \cite{miotto2022gpt3} reported that GPT-3’s personality profile fluctuates with the adjustment of temperature values in the model's settings. \cite{song2023large} observed \textcolor{red}{inherent biases} within LLMs, leading to a tendency to produce identical answers irrespective of the situational context being tested.

Building upon these insights, \cite{serapiogarcía2023personality} has underscored the significance of testing various model versions and sizes, employing a larger parameter volume, and leveraging Supervised Fine-Tuning techniques to augment the reliability of personality assessments in LLMs.

\subsubsection{Validity}

The discussion on the validity of personality assessments for Large LLMs is also not marked by a consensus. \cite{jiang2023evaluating} incorporated a validity assessment by prompting LLMs to explain the reason for selecting particular options within Likert-scale personality questionnaires. The responses successfully indicated that LLMs displayed a strong understanding of the question items, highlighting their research validity. Nonetheless, upon conducting an exhaustive analysis of the responses from LLMs to personality questionnaires, researchers fail to discern patterns that were both intended in the design and observed in human subject pools \cite{dorner2023personality}. In conclusion, before conducting personality assessments for LLMs, validity cannot be assumed without a thorough and critical analysis.


\subsection{Findings and Open Challenges}
We summarize the findings in the literature by answering the previously raised questions.

% \cite{miotto2022gpt} rephrases the items in the HEXACO questionnaire into the third person plural as the prompts and asks GPT-3 to answer the extent of how much the descriptions are similar to itself. The overall scores obtained from GPT-3 are then compared with the HEXACO scores of human participants. Although no significant results show that GPT-3 demonstrates an entirely consistent response pattern of personality, They concluded that GPT-3's personality varies with temperature. Therefore, anyone employing GPT-3 as a test subject should familiarize themselves with the personality traits relevant to the study at a given temperature and choose accordingly.

% \cite{li2023does} utilize zero-shot prompting to evaluate personality traits and implicit dark personality patterns of LLMs with the Big Five Inventory (BFI) and the Short Dark Triad (SD-3).  They first rephrase each question in the personality inventories as prompts for LLMs and then define a rule-based function that identifies the selected option and the corresponding score in the answer of LLMs. The experiments show that even after being instruction fine-tuned with several safety metrics, some LLMs (GPT-3, InstructGPT, and Flan-T5-XXL) scored higher than humans in negative personality traits. 

% \cite{jiang2023evaluating} construct the Machine Personality Inventory (MPI) datasets upon psychometric inventories \cite{goldberg1999broad, goldberg2006international, johnson2005ascertaining, johnson2014measuring, lang2011short}. They define each test item within MPI as a multiple-choice question and conduct zero-shot prompting for LLMs to assess their personalities exhibited.

% \cite{safdari2023personality} used prompts to instruct models to rate items from each psychometric test \cite{john1999big,goldberg1999broad} on a standardized response scale and then rigorously evaluated the psychometric properties of LLM responses through a suite of statistical analyses of reliability and construct validity. The LLM personality measurements were reliable for medium (around 62B) and large (around 540B) instruction fine-tuned LLM; while the construct validity of the personality assessment is positively related to the model size and the instruction fine-tuning.

% \cite{huang2023chatgptMBTI} assesses the personality of multiple LLMs by prompting questions of the MBTI test in different orders, and languages. They found OpenAI GPT family (\textit{e.g.}, ChatGPT,  text-davinci-003, and GPT-4) maintain a similar personality trait identified as ENFJ across MBTI tests in different question orders and languages.

% \cite{huang2023revisiting} examines the reliability of psychological scales initially designed for human assessment
% when applied to LLMs. The findings demonstrate that gpt-3.5-turbo can represent diverse personalities by adjusting prompt inputs.
% This study aims to determine the reliability of applying personality assessments to LLMs, explicitly investigating whether LLMs demonstrate consistent personality traits. 

% To comprehensively assess the psychological portrayal of LLMs, 
% \cite{huang2023chatgpt} developed PsychoBench, a benchmarking framework containing three widely-recognized personality scales (Big Five Inventory (BFI) \cite{john1999big}, Eysenck Personality Questionnaire (Revised) (EPQ-R, \cite{eysenck1985revised}), and Dark Triad Dirty Dozen (DTDD) \cite{jones2014introducing}) and scales in other domains. The authors instructed LLMs to reply only a number within the Likert scale levels of the questions in the personality scales. The result scores of LLMs are compared with the results of human beings. They found that different LLMs exhibit distinct personality traits and LLMs generally exhibit more negative traits than human norms, similar to the findings in \cite{li2023does}.

% \cite{pan2023llms} prompted LLMs with 93 questions to obtain the MBTI test scores by analyzing their responses. LLMs exhibit different MBTI personality types. However, after instruction fine-tuning, LLMs' personality traits exhibited can be easily changed by prompting.

% \cite{wang2024incharacter} introduces a novel perspective to evaluate the personality fidelity of RPAs with psychological scales

% \cite{romero2023gpt} Our study aims to determine the reliability of applying personality assessments to LLMs, explicitly investigating whether LLMs demonstrate consistent personality traits. 


% \cite{song2023large} find that many LLMs personality test responses do not preserve option-order symmetry.

% \cite{dorner2023personality} provide evidence that LLMs’ responses to personality tests systematically deviate from typical human responses, implying that these results cannot be interpreted in the same way as human test results.


% \cite{sorokovikova2024llms} The Big5 personality profiles of GPT4, Llama2, and Mixtral, as elicited through the IPIP-NEO-120 questionnaire, demonstrate the models’ differing propensities for specific traits. 

% \cite{shu2024dont} reveals that even simple perturbations significantly downgrade a model’s question-answering ability and that most LLMs have low negation consistency. Our results suggest that the currently widespread practice of prompting is insufficient to accurately and reliably capture model perceptions,

% \cite{lacava2024open} conduct MBTI tests on different LLMs and found each Open LLM agent showcases distinct human personalities;


% \cite{frisch2024llm} Do persona-conditioned LLMs show consistent personality and language use in interaction? In this study, we explore the capability of GPT-3.5 agents conditioned on personality profiles to consistently express their assigned traits in interaction, using both explicit and implicit personality assessments. Conclusion: LLM agents can be shaped to mimic human personality profiles

% \cite{digman1990personality} and subsequently classifies the text responses into the big five personality traits using a Zero-shot classifier. The results indicated noticeable variations in trait distributions of text generated using different language models. Interestingly, by investigating the personality traits of the pre-training datasets of LLMs through text classification for sub-samples, the authors also validated their hypothesis: language models generate text responses that reflect the personality traits of the datasets they were trained.

% Similar to \cite{karra2022estimating}, \cite{pellert2022ai} also assumed that LLMs inadvertently yet inevitably, acquire psychological traits from the vast text corpora on which they are trained. They prompted the questions from personality inventories recorded the language models' responses and conducted zero-shot classification to obtain their personality scores. The results indicate that seldom language models possess an extreme, accentuated personality and most models score low dark traits. However, it is worth mentioning the models they assessed are not large-scale generative models like GPT-3, GPT-4, or ChatGPT. So, the results here are also not suitable for the state-of-the-art LLMs.


% \cite{hilliard2024eliciting} use a novel elicitation approach using prompts derived from common interview questions, as well as prompts designed to elicit particular Big Five personality traits to examine whether the models were susceptible to trait-activation like humans are, to measure their personality based on the language used in their outputs



% \subsection{Are self-assessment results for LLMs reliable?}

% \subsubsection{Findings 2}: 







% ----------














==> Inducing_Personality.tex <==
\section{LLM's Personality Exhibition}

With the enhancement of conversational abilities of LLMs, the capacity to exhibit diverse personalities is crucial for LLMs to satisfy users' needs in various application scenarios \cite{jiang2023evaluating}. For example, we may prefer chatbots that are outgoing and not anxious, while an emergency service bot should be responsible when providing recommendations. Besides, enabling LLMs to alter their personality traits over time in response to changing environmental factors would result in dynamic AI systems that better align with users' changing needs and preferences, ultimately enhancing the user experience \cite{karra2022estimating}. 

More importantly, pioneering studies \cite{gehman2020realtoxicityprompts,bender2021dangers,bommasani2021opportunities,tamkin2021understanding} observe that LLMs are prone to generate potentially harmful or inappropriate content due to unavoidable toxic information in pre-training datasets. Effectively modifying the personality traits of LLMs provides a nuanced method to decrease the probability of generating toxic content by shaping the tone, style, and substance of the resulting text \cite{li2023does}. 

\subsection{Problem Definition}

To summarize the requirements in the described scenarios above, LLM's personality exhibition can be defined as \textbf{How to control LLMs to reflect the specified personality traits in the generated text content?}
Approaches to solving this problem are categorized into two classes: 
\textbf{Editing}, which involves modifying the model parameters of LLMs to alter the potential intrinsic personality of LLMs acquired from pre-training; and \textbf{Inducing}, which fixes the original LLM but utilizes prompt engineering to induce LLMs to exhibit specific personalities.

\subsection{Editing LLM's Personality}
One straightforward method for shaping the personalities of LLMs is altering the model parameters through continual pre-training or fine-tuning on specific corpora. This approach inherits from the text style transfer/control research on pre-trained language models, where the emphasis was on manipulating the stylistic elements such as sentiment, tone, or demeanor of textual output \textcolor{red}{(add some citations)}.
\cite{pan2023llms} conduct continual pre-training on LLMs with distinct corpora, finding that the type of training corpus (\textit{e.g.}, wiki, question-answering, or examination materials) can affect the MBTI type exhibited by LLMs, especially in the dimensions of T/F and J/P.  While \cite{karra2022estimating} proposed to alter the personality traits of LLMs (GPT-2) by fine-tuning with additional personality-annotated text data with or auxiliary text classification or generation tasks. Similarly, \cite{liu2024dynamic} constructed a personality-dialogue dataset to fine-tune LLMs on the task of generating dialogue content aligned with specified personality traits, assessed by GPT-4. Both methods show that fine-tuning can effectively modify the personality traits of LLMs. However, it is also suggested that may inadvertently affect non-focal traits, potentially leading to unintended personality exhibition. 

Besides continual pre-training and traditional fine-tuning, instruction fine-tuning (\textcolor{red}{citation}) also gains a lot of attention in editing LLM's personality. Instruction fine-tuning is originally designed to improve the capacity of LLMs to follow human instructions for performing different tasks through fine-tuning on various question-answering pairs. Under the context of editing LLM's personality, researchers also facilitate it to control LLMs to exhibit specified personality traits.
\cite{li2023does} conducted instruction fine-tuning to GPT-3 using questions from the BFI questionnaire and their corresponding answers indicating higher \textit{agreeableness} and lower \textit{neuroticism}. Their approach resulted in a more positive and emotionally stable personality exhibition.
Besides utilizing the questionnaires, \cite{cui2023machine} construct the Behavior dataset by employing ChatGPT to classify each instruction in the original Alpaca dataset into the most fitting MBTI dimension out of the four. They then fine-tune LLMs with the dataset to respond to general user instructions consistently with specific personality traits. Similarly, \cite{mao2024editing} leveraged GPT-4 to generate question-answering pairs in specific scenarios facilitated by psychology domain knowledge for instruction fine-tuning LLMs. Furthermore, they employed a variety of baseline methods for pre-personality editing on their constructed dataset.

It is noteworthy that the majority of the aforementioned fine-tuning methods employ parameter-efficient fine-tuning techniques, utilizing either LoRA \cite{mao2024editing,cui2023machine,liu2024dynamic} or adapter modules \cite{liu2024dynamic}. This approach allows for the modification of a very small subset of LLMs' parameters to achieve the desired results.


\subsection{Inducing LLM's Personality}

While the aforementioned methods have demonstrated partial effectiveness, editing the personality of LLMs through parameter adjustment still relies on computational resources and dataset construction. An alternative method that is more widely applied and more efficient involves fixing the parameters of the LLM and employing prompting techniques to induce LLMs to exhibit specific personalities. Following existing research \cite{pan2023llms}, we categorize the inducing methods into Explicit Prompting, which utilizes the explicit description or definition of a specific personality as the instruction; and Implicit Prompting, which leverages demonstrative examples of how the specified personality is implied in various scenarios as the input prompts in an in-context learning manner. \\

\noindent
\textbf{Explicit Prompting}: 
According to the lexical hypothesis of personality (\textcolor{red}{add citation}), personality is defined by the descriptive words of humans.
Numerous researchers \cite{jiang2023evaluating, safdari2023personality, weng2024controllm, stockli2024personification} adopt descriptive adjectives of personality traits from psychological findings as the prompt content to elicit personality exhibition in LLMs. Although these adjectives can precisely describe specified personality traits, they struggle to provide detailed guidance on exhibiting specific personalities. Concurrently, there are also studies \cite{pan2023llms, tan2024phantom, huang2023chatgptMBTI, lacava2024open, jiang2023personallm, kovac2023large} leveraging natural sentences to describe the concrete manifestations of specified personalities across various aspects or employing the interpretations of personality from psychological questionnaires \cite{noever2023ai}. Nevertheless, due to the sensitivity of LLMs to prompting cues (\textcolor{red}{add citation}), the efficacy of such methods is also affected by factors such as the content quality, or the phrasing of the prompts.\\

\noindent
\textbf{Implicit Prompting}: While explicit prompting offers a clear description of personality, it struggles to provide precise guidance on how personality is manifested in specific application scenarios. The most straightforward way to find examples for implicit prompting is adopting question-answering pairs derived from personality questionnaires \cite{pan2023llms,huang2023chatgptMBTI,klinkert2024driving}, wherein multiple questions encapsulate the manifestations or preferences of personality across a variety of potential scenarios. Besides, researchers also employ demographics or profiles of typical individuals with the specified personalities as examples to guide LLMs in exhibiting the inherent personalities \cite{huang2023chatgptMBTI,he2024afspp,petrov2024limited}. Furthermore, there are studies that use concrete examples of personality exhibitions in specific contexts, such as restaurant reviews \cite{ramirez2023controlling} or behaviors on social networks \cite{he2024afspp}, as examples to facilitate guidance.


\subsection{Findings and Open Challenges}
In addition to reviewing the various methods for LLMs' personality exhibition presented in existing works, we also summarize their main findings and the unresolved open challenges, shown as follows.

\subsubsection{Findings:} 

\noindent
\textbf{1. Which method is more effective for controlling LLMs to exhibit specific personalities?} First, due to the variety of different methods and datasets applied to distinct LLMs, it is challenging to deduce a universal solution to which approach is more effective. However, faced with extensive parameters of LLMs, inducing appears to be a more practical strategy. Moreover, some studies (\textit{e.g.,} \citet{mao2024editing}) have demonstrated that inducing methods outperform the editing methods across most metrics on the same LLMs. Besides these two mainstream methods, researchers \cite{li2024tailoring} also attempt to control LLMs' personality exhibition by influencing the probability distribution in decoding. \\

\noindent
\textbf{2. Among existing work, what is the performance of LLMs' personality exhibition?} Precisely controlling an LLM to exhibit a composite personality is a relatively challenging task \cite{lacava2024open, safdari2023personality}. However, researchers \cite{huang2023chatgptMBTI} show that modifying only certain single dimensions or facets of personality is more feasible. \\

\subsubsection{Open Challenges:} 

\textbf{Exhibition Inconsistency:} Despite most existing studies have validated the effectiveness of their personality exhibition approaches through questionnaires or response analysis, some studies \cite{ai2024cognition} indicate a misalignment between the induced personality traits in the evaluation and those exhibited in real-world scenarios. This highlights the need for more context-aware evaluations to ensure consistent personality expression in real-world applications. \\

\noindent
\textbf{Exhibition Stability:} The use of natural language induction has been proven effective in influencing the expression of personality traits in LLMs. However, during user interactions, the personality exhibited by the LLM may also be influenced by the dialogue context. Although many LLMs employ system-level prompts or safeguarding policies to prevent their responses from being affected by user inputs, maintaining stability in personality exhibitions during interactions remains an open challenge.





% \subsection{Applications}

% ...



%\cite{safdari2023personality}: We evaluated LLM personality score changes in response to personality-shaped prompts across two experiments: single trait shaping and multiple trait shaping
%
%(1) Quantifying how strongly shifts in IPIP-NEO score distributions were related to shifts in targeted trait levels embedded in our prompt sets (i.e., through Spearman's rank correlation coefficient.
%
%(2) Inspecting the distance between personality score distributions obtained in response to our most extreme prompt sets; specifically, the set of prompts we shaped to be the lowest possible levels of a trait (versus those shaped to be the highest possible levels of a trait) should result in distributions of scores that are farther away from each other.
%
%\cite{karra2022estimating} calculate the personality score of the generated text by modified LLM through zero-shot personality classifiers.












==> Inducing_Personality_haoming.tex <==
\section{LLM's Personality Exhibition}

With the enhancement of conversational abilities of LLMs, the capacity to exhibit diverse personalities is crucial for LLMs to satisfy users' needs in various application scenarios \cite{jiang2023evaluating}. For example, we may prefer chatbots that are outgoing and not anxious, while an emergency service bot should be responsible when providing recommendations. Besides, enabling LLMs to alter their personality traits over time in response to changing environmental factors would result in dynamic AI systems that better align with users' changing needs and preferences.\cite{karra2022estimating}  Personalized agent models can tailor their expression of personality patterns based on user preferences, making it closely aligned with user habits.\cite{li2024tailoring}This ultimately enhances the overall user experience.
%这里加了一句话(1)：\cite{li2024tailoring}


More importantly, pioneering studies \cite{gehman2020realtoxicityprompts,bender2021dangers,bommasani2021opportunities,tamkin2021understanding} observe that LLMs are prone to generate potentially harmful or inappropriate content due to unavoidable toxic information in pre-training datasets. Effectively modifying the personality traits of LLMs provides a nuanced method to decrease the probability of generating toxic content by shaping the tone, style, and substance of the resulting text \cite{li2023does}. 

\subsection{Problem Definition}
To summarize the requirements in the described scenarios, LLM's personality exhibition can be defined as: \textbf{Developing strategies to modify the LLM's parameters or the response generation mechanism to reflect the desired personality trait in the generated content.}

% 加入“其他方法”？
As the personalities of LLMs may originate from the corpus fed to the model during training, approaches to solving this problem are categorized into two classes: \textbf{Editing}, which involves Supervised Fine-tuning (SFT) for LLMs using specific corpora to guide LLMs exhibiting specific personality traits; and \textbf{Inducing}, which utilizes prompt engineering to induce specific personalities in LLMs embedded from pre-training data.

% 加入对tuning的分类描述
\subsection{Editing LLM's Personality}
Editing the personalities of the language models can be viewed as updating the model's parameters such that it generates modified text responses that are closer to the desired personality traits \cite{karra2022estimating}. Therefore, existing studies explored whether the personalities can be edited after training/fine-tuning with different corpora.

\cite{karra2022estimating} proposed to alter the personality traits of language models (GPT-2) with additional personality-annotated text data by text generation tasks or auxiliary text classification tasks. They demonstrated that finetuning can effectively alter the personality traits of language models like GPT-2 by allowing them to learn from a new data corpus. However, they also found that finetuning can change the personality scores of other traits besides the focal trait, which may be undesirable if precise control over a specific trait improvement is required.

\cite{li2023does} used question-answer pairs of BFI for instruction fine-tuning, resulting in a model with a more positive and stable personality. Specifically, they first collected the BFI answers from their previous experiments on LLMs. Then, they defined the results in which the score on agreeableness is higher and the score on neuroticism is lower than the human average as positive answers. Finally, they construct 3,916 question-answer pairs from the positive answers to instruction fine-tune the LLMs. After the instruction fine-tuning, the model exhibited a more positive and stable personality.



%把这些写了
\cite{cui2023machine}

\cite{mao2024editing}

\cite{li2024evaluating}
%这是同一篇？？

\cite{pan2023llms}

% 加入对inducing的分类描述
\subsection{Inducing LLM's Personality}

\cite{lacava2024open} personality-conditioned prompting produces varying effects on the agents, with only few successfully mirroring the imposed personality, while most of them being “closedminded” (i.e., they retain their intrinsic traits);



When the model size is too large to be readily adapted, prompting becomes more applicable compared to fine-tuning \cite{liu2023pre}. Besides, prompts enable zero-shot in-context learning, resulting in generalizable controlling beyond fine-tuning. So, researchers also investigate to design prompts to induce specific personalities in LLMs embedded from pre-training data.

\cite{huang2023chatgptMBTI} employed several prompting approaches to control the personality of LLMs, directly assigning a personality to ChatGPT with a prompt describing the personality \cite{santurkar2023whose}, inducing the atmosphere within the prompt context to influence ChatGPT's personality, and instructing ChatGPT to play the role of a persona with a predetermined personality. They found that precisely modifying ChatGPT's personality remains an unresolved challenge. However, it is relatively feasible to change just from Extroverted to Introverted.

\cite{jiang2023evaluating} devised an automatic prompting method, PERSONALITY PROMPTING ($P^2$) to induce the specified personality trait in the LLM. In detail, they proposed to first construct a human-designed naive prompt for a specified personality trait. Then, the naive prompt is transformed into a keyword prompt with trait descriptive words derived from psychological studies. They self-prompt the target LLM with the keyword prompt to generate short descriptive sentences of the specified trait to invoke its internal knowledge to exhibit the trait.

\cite{safdari2023personality} devised a novel prompting methodology that shaped each personality trait of the big five personality traits at nine intensity levels, using Likert-type linguistic qualifiers and trait adjectives. Besides, they also tested the abilities of LLMs to shape synthetic Big Five traits concurrently, specifying target levels of all five dimensions in every prompt set at the same time.  We successfully shaped personality traits in LLMs independently and concurrently, in single- and multitrait shaping experiments, respectively, particularly in larger models, \textit{e.g., Flan-PaLM 540B \cite{chung2022scaling}}.

\cite{jiang2023personallm} had GPT-3.5 assume hundreds of personas by prompting it to behave with different combinations of personality traits, where the prompts are adopted from the questions in a personality inventory \cite{john1999big}. 

\cite{pan2023llms} design two types of prompts to guide the models in an in-context learning manner: 1) Explicit prompt: role-playing, which provides a detailed description of a specific role to be played (\textit{e.g., You possess an outgoing personality, enjoy envisioning innovative concepts, and possess a strong inclination towards spontaneity and improvisation...}). 2) Implicit prompt: few-shot questions-answer pairs (\textit{e.g., Do you prefer? A. Be alone, B. With friends. Answer: B}). Both results show that the interference of zero-shot prompting has minimal impact on LLMs for questionnaire personality tests. However, they also concurrently demonstrated that for models like ChatGPT, which have undergone instruction fine-tuning, the effectiveness of personality modification with prompts can be improved. Moreover, this study also empirically validated that training LLMs on different corpora can indeed alter the exhibited personality to a certain extent, especially in the dimensions of Thinking/Feeling and Judging/Perceiving. 



\subsection{Findings and Open Challenges}

The most commonly used method for assessing the effectiveness of personality exhibition in LLMs is evaluating changes in quantitative personality scores. However, due to the variety in psychological inventories adopted by different existing studies,  (1) facets measured by different personality inventories are different; (2) personality scores calculated by different inventories are also different; (3) more importantly, approaches of inducing or editing personality is highly related to the inventories. Consequently, impartially comparing the effectiveness of methods for exhibiting specific personalities remains a significant challenge.

%\cite{safdari2023personality}: We evaluated LLM personality score changes in response to personality-shaped prompts across two experiments: single trait shaping and multiple trait shaping
%
%(1) Quantifying how strongly shifts in IPIP-NEO score distributions were related to shifts in targeted trait levels embedded in our prompt sets (i.e., through Spearman's rank correlation coefficient.
%
%(2) Inspecting the distance between personality score distributions obtained in response to our most extreme prompt sets; specifically, the set of prompts we shaped to be the lowest possible levels of a trait (versus those shaped to be the highest possible levels of a trait) should result in distributions of scores that are farther away from each other.
%
%\cite{karra2022estimating} calculate the personality score of the generated text by modified LLM through zero-shot personality classifiers.












==> Personality_Recognition.tex <==
\section{Personality Recognition in LLM}
Beyond assessing the potential personality traits inherent in LLMs and enabling them to exhibit specific personalities, there is also a growing interest among researchers to explore whether LLMs identify the personality of individuals. 

Personality recognition holds significant importance in the social sciences and can lead to numerous applications; within the field of Computer Science, it is also a longstanding research issue. It has evolved from the early identification of statistical features in daily conversations and social behavior habits to leveraging the deep semantic understanding capabilities of Neural Networks (NN) to comprehend social media posts, self-report essays, or conversation content. However, due to privacy concerns and the professional nature of personality analysis, obtaining sufficient personality annotations for model training has always been a significant challenge. With the advent of LLMs, their exceptional few-shot and zero-shot capabilities have, to some extent, mitigated the issue of limited availability of labeled data. Empirical evidence from the majority of studies has shown that employing LLMs for personality recognition can achieve better results than traditional NN models. Besides, as LLMs are able to generate explanations for identifying personality traits, the interpretability of the results is also substantially enhanced. 

\subsection{Problem Definition}

We formally define Personality Recognition in LLMs as \textbf{How to categorize the personality traits exhibited in the given text content?} Existing research on personality recognition in LLMs is primarily divided into two aspects: \textbf{Personality Recognition by LLMs}: exploring the zero-shot capabilities of LLMs for personality recognition, and  \textbf{LLM-enhanced Personality Recognition}: utilizing LLMs to enhance other personality recognition models. Below, we will introduce these two categories of work separately.

\subsection{Personality Recognition by LLMs}

Benefitting from the robust zero-shot capabilities of LLMs in NLP tasks, some studies directly utilize text content, such as social media posts \cite{ganesan2023systematic,peters2023large}, written documents \cite{ji2023chatgpt,derner2023chatgpt}, or daily conversation \cite{peters2024large} as the input prompts to LLMs for personality recognition. Without additional training or fine-tuning, LLMs indeed exhibit impressive personality recognition ability and can provide natural language explanations through text-based logical reasoning \cite{ji2023chatgpt}. Furthermore, it is also suggested that mimicking a user's acquaintance can enhance LLMs' personality recognition performance in the conversation scenarios\cite{peters2024large}. Beyond traditional text-based personality recognition, researchers also integrated transcripts of video data as inputs for LLMs to enable the processing of personality recognition in more diverse contexts \cite{amin2023will,10463124}, thereby corroborating the personality recognition capabilities of LLMs.

In addition to directly employing text content for personality recognition as prompts for LLMs, some researchers have also explored LLMs' comprehension of personality questionnaires for personality recognition. \cite{rao-etal-2023-chatgpt}  investigate the ability of ChatGPT and its variants to assess human personalities based on MBTI questionnaires by designing a series of prompting techniques to rephrase MBTI questions and observe how LLMs correlate questionnaire responses with underlying personality traits. They show that LLMs undergone RLHF have much better performance. Besides, researchers \cite{yang2023psycot} also attempt to prompt LLMs with the items from the personality questionnaire in a chain-of-thought manner, emulating the way individuals complete psychological questionnaires in multi-turn dialogues. Their method is validated to significantly improve the performance and robustness of GPT-3.5 in personality recognition.

\subsection{LLM-enhanced Personality Recognition}

Although LLMs are validated to easily outperform traditional NN models and pre-trained language models on personality recognition in a zero-shot manner, most LLMs still underperform models that are specially trained for personality recognition \cite{ji2023chatgpt,ganesan2023systematic,amin2023will}. Therefore, researchers also attempt to use LLMs to enhance existing personality recognition models by augmenting the input data \cite{hu2024llmvssmall,wen2024affective,amin2023chatgpts} or providing additional recognition features \cite{cao2024large}, especially in the shortage of annotated data.

For example, when using traditional NN models to identify personality traits from social media posts, LLMs can generate additional analysis on these posts, in the aspects of semantic, sentiment, and linguistic as augmentation \cite{hu2024llmvssmall}. Furthermore, LLMs can be utilized to generate semantic interpretations of personality classification labels. In the context of personality recognition in conversations, LLMs can also be engaged in affective analysis of the utterances, leveraging the correlation between affective information and personality to provide additional cues for personality recognition \cite{wen2024affective}. Moreover, the personality analysis and interpretation generated by ChatGPT about the given text can serve as features to assist machine learning models in personality recognition \cite{amin2023chatgpts}. Due to the rich information encapsulated within the embeddings during pre-training, even the word embeddings from GPT-3 for names of well-known figures can contribute to analyzing their personality traits \cite{cao2024large}.

\subsection{Findings and Open Challenges}

We summarize the findings and open challenges uncovered by the above studies as follows:\\


\subsubsection{Findings}
% \noindent
% \textbf{Finding 1:} With limited annotated data, LLMs outperform traditional models in personality recognition but still lag behind SOTA, making them unsuitable for direct use in practical applications.
\noindent
\textbf{1. Can we directly apply LLMs for personality recognition?} With limited annotated data, LLMs, especially those refined by RLHF, exhibit superior performance in personality recognition but still underperform the specialized SOTA models. Therefore, in practical applications, LLMs without specialized training and fine-tuning are not suitable for directly obtaining results in personality recognition. \\

\noindent
\textbf{2. How can LLMs facilitate existing personality recognition models?} LLMs can be utilized to provide additional information, such as explanations of the input, and classification features, to facilitate traditional personality recognition models. \\

\subsubsection{Open Challenges}

\noindent
\textbf{Demographic Biases:} Despite the impressive performance in personality recognition, LLMs also exhibit potential biases towards certain demographic attributes (\textit{i.e.}, the recognition performance of certain genders and ages is better than others), suggesting a potential systematic bias stemming from the underlying training data or differences in online self-expression \cite{ji2023chatgpt,peters2023large}. \\

\noindent
\textbf{Positivity Biases:} As most LLMs are refined by RLHF to align with human preferences, they tend to assign socially desirable scores across key personality dimensions to the input. This propensity may render the results less authentic and convincing \cite{derner2023chatgpt}. \\




% The zero-shot prompting ability of LLMs has been shown to easily outperform traditional neural network models as well as some pre-trained language models \cite{ji2023chatgpt,10463124,peters2023large}.



% However, there exists a potential for biases towards certain demographic attributes, which has been observed in several evaluations \cite{ganesan2023systematic,peters2023large}. 
% It is noteworthy that LLMs that have undergone Reinforcement Learning with Human Feedback (RLHF) exhibit a much-improved performance \cite{rao-etal-2023-chatgpt}. Nonetheless, when compared to specialized personality recognition models, LLMs under zero-shot prompting may still underperform, highlighting the need for further refinement and training in this domain \cite{ji2023chatgpt,ganesan2023systematic,amin2023will}.

% \cite{ganesan2023systematic} performed a systematic investigation of GPT3's zero-shot ability on personality estimation through social media posts. The study revealed that simple and directly querying LLMs did not elicit robust performance, while the integration of trait-specific knowledge in prompts can significantly enhanced the results. Even so, zero-shot LLM still falls short of the extensively supervised personality recognition model.

% \cite{ji2023chatgpt} evaluates ChatGPT's zero-shot performance on text-based personality recognition tasks. The authors employed different prompting strategies, including zero-shot prompting, zero-shot Chain-of-Thought (CoT) prompting, one-shot prompting, and a level-oriented prompting strategy combining text prompts in different levels (word, sentence, or document). Their results show that zero-shot prompting ChatGPT can easily outperform traditional NN models and pre-trained language models (RoBERTa). Nevertheless, there remains a substantial disparity between ChatGPT and a state-of-the-art specialized personality recognition model. Besides, the researchers also found that ChatGPT exhibited some biases towards certain demographic attributes. For example, women were more likely to be associated with high levels of Openness, Conscientiousness, and Agreeableness compared to men. This may lead to unfair treatment.

% Similarly, \cite{rao-etal-2023-chatgpt} presents a framework for evaluating the ability of ChatGPT and its variants to assess human personalities based on MBTI questionnaires. Specifically, they designed a series of prompting techniques to rephrase MBTI questions and observe how LLMs correlate questionnaire responses with underlying personality traits. The authors evaluated the consistency (the reliability of assessments across multiple tests), the robustness (how stable LLMs perform under varied prompt wordings), and the fairness (differences for biases across different demographic groups), of LLMs' performance. The results show that ChatGPT and GPT-4, (\textit{i.e.}, LLMs undergone Reinforcement Learning from Human Feedbacks (RLHF)), surpass InstructGPT across all aspects.

% \cite{10463124} explored measuring interviewees' personalities with LLMs in Asynchronous Video Interviews (AVIs). The interview questions and the transcribed responses are provided to LLMs for personality analysis. They also employed a chain-of-thought prompting strategy, requiring LLMs to not only rate the interviewee's personality but also explain the reasoning process. The results show that LLMs can achieve competitive results in zero-shot predicting personality traits. However, they also suffered from uneven performance across different traits, insufficient test-retest reliability, and the emergence of certain biases.

% \cite{amin2023will} employed ChatGPT to analyze the transcripts of vlogs \cite{ponce2016chalearn} for personality classification with simple prompts in a zero-shot manner. In terms of personality trait assessment, ChatGPT performs worse than the three baseline models on all traits. Although ChatGPT is a general model that can perform well on a variety of problems without special training, its performance is not as good as models trained specifically for downstream tasks.

% \cite{peters2023large} assessed the ability of GPT-3.5 and GPT-4 to derive the Big Five personality traits from users' Facebook status updates in a zero-shot learning scenario. The authors demonstrated the capacity of LLMs to derive psychological profiles from social media data, even without specific training. However, their results also suggest biases in personality inferences with regard to gender and age, \textit{i.e.}, results for women and younger individuals are more accurate.

% To utilize the potential reasoning ability in LLMs for personality recognition, \cite{yang2023psycot} prompts LLMs the items from the personality questionnaire in a chain-of-thought manner, mimicing the way individuals complete psychological questionnaires in multi-turn dialogues. Their method is valided to significantly improve the performance and robustness of GPT-3.5 in personality recognition


% By summarizing the above-introduced studies, we observed several findings:

% 1. ChatGPT has some ability, but cannot outperform the supervised model \cite{amin2023will,peters2023large}

% 2. Most LLMs have intrinsic bias. a potential systematic bias stemming from the underlying training data or differences in online self-expression \cite{peters2023large}.


% \subsection{How to apply LLMs Recognize Personality?}

% To distill the useful knowledge from the LLMs for personality detection, \cite{hu2024llmvssmall} employ LLM to generate the analyses of the input user posts from the aspects of semantic, sentiment, and linguistic to augment the input data. Besides, they also utilize the LLM to enrich the information of personality labels for enhancing the detection performance.


% To achieve interpretable personality recognition in daily conversation scenarios, \cite{10494487} adopt text descriptions of personality labels from psychology findings as the auxiliary input and formulate personality recognition as a natural language inference (NLI) problem for LLMs. 

% .


% \subsubsection{Findings}
% 1. it can indeed reduce the annotation shortage issue
% 2. most of them are prompt engineering, utilizing LLM to generate additional information


% \subsection{Discussions}


% \begin{itemize}
% 	\item most of them are just prompting engineering
% 	\item The study observed that ChatGPT's analysis showed biases towards certain groups, \textit{e.g.}, gender, age, occupations, and education degrees, which could lead to unfair treatment. 
% 	\item When assessing the personality of specific individuals, LLMs generated uncertain answers due to a lack of personal background information, highlighting the need for richer context or fine-tuning. \cite{rao-etal-2023-chatgpt}
% \end{itemize}


==> Resources.tex <==
\section{Resources}






\begin{table*}[h]
\centering
\scriptsize
% \linespread{1}
\renewcommand{\arraystretch}{1.2}
% \begin{tabular}{m{4cm}m{4cm}cm{5cm}}
\begin{center}
\begin{tabular}{|p{3cm}|p{4cm}|m{4cm}|m{4cm}|}
% \toprule
\hline
\textbf{Dataset} & \textbf{Types} & \textbf{Descriptions} & \textbf{Download Links} \\
\hline
\cite{bodroza2023personality}\break Open Science Framework repository & Self-assessment & Questionnaires includes Self-Consciousness Scales, BFI, HEXACO-100, Short Dark Triad and others& \href{https://osf.io/2k458/?view_only=6886694c6f8449488cfbc4e8f78ea2b0}{https://osf.io/2k458/?view\_only=\break 6886694c6f8449488cfbc4e8f78ea2b0} \\
\hline
PsychoBench \break \cite{huang2023chatgpt} &  Self-assessment &  Psychological scales covering personality traits, interpersonal relationships, motivational tests, and emotional abilities & \href{https://github.com/CUHK-ARISE/PsychoBench}{https://github.com/CUHK-ARISE/PsychoBench} \\
\hline
MODEL-PERSONAS \break \cite{shu2024dont} & Self-assessment & 39 different persona measurement instruments, standardized into 693 questions across 115 persona axes. & \href{https://github.com/orange0629/llm-personas/tree/master/data}{https://github.com/orange0629/llm-personas/tree/master/data}\\



\hline
\cite{miotto2022gpt} & Self-assessment & HEXACO scale and Human Values Scale & \href{https://github.com/ben-aaron188/who_is_gpt3}{https://github.com/ben-aaron188/who\_is\_gpt3} \\




\hline
Ten Item Personality Inventory \break \cite{romero2023gpt} & Self-assessment & TIPI questionnaires across different linguistic environments & \href{https://osf.io/bf5c4/?view_only=f870d9e7258a4c2bb4430952f985b196}{https://osf.io/bf5c4/?view\_only=\break f870d9e7258a4c2bb4430952f985b196} \\

\hline
\cite{pellert2023ai} & Self-assessment & BFI and Short Dark Tetrad questionnaire in German and English& \href{https://github.com/maxpel/psyai_materials/tree/master/44_items_big5}{https://github.com/maxpel/psyai\_materials \break /tree/master/44\_items\_big5} \\



\hline
\cite{dorner2023personality} & Self-assessment & 50-item IPIP Big Five Markers and BFI 2 questionnaire & \href{https://openpsychometrics.org/tests/IPIP-BFFM/}{https://openpsychometrics.org/tests/IPIP-BFFM/}\\

\hline
\cite{stockli2024personification} & Self-assessment& Dataset include the HEXACO Personality test, the Dark Triad test and Others &\href{https://github.com/AdritaBarua/2024-Psychology-of-GPT-4}{https://github.com/AdritaBarua/2024-Psychology-of-GPT-4}\\

\hline
\cite{ai2024cognition} & Self-assessment &BFI-44 as a self-report measure providing detailed insights into the Big Five traits &\href{https://www.ocf.berkeley.edu/~johnlab/bfiscale.php}{https://www.ocf.berkeley.edu/~johnlab/bfiscale.php}\\

\hline
\cite{ai2024cognition} & Self-assessment &The TDA-100 for its checklist format that aligns with the Big Five
dimensions&\href{https://ipip.ori.org/newNEODomainsKey.htm}{https://ipip.ori.org/newNEODomainsKey\break .htm}\\

\hline
\cite{ai2024cognition} & Self-assessment &16 Personalities questionnaire offers an accessible and engaging way to explore MBTI types.&\href{https://www.16personalities.com}{https://www.16personalities.com}\\

\hline
Kaggle MBTI \break \cite{song2024identifying} & Self-assessment &The Kaggle MBTI Dataset containing 8675 records, each corresponding to an individual's MBTI type, and includes excerpts from the individual's last 50 posts or comments on the PersonalityCafe forum used to fine-tune a Llama2-7B model.&\href{https://www.kaggle.com/datasets/datasnaek/mbti-type}{https://www.kaggle.com/datasets/datas\break naek/mbti-type} and \href{https://www.personalitycafe.com/forums/myers-briggs-forum.49}{https://www.personalitycafe.com/forums/\break myers-briggs-forum.49}\\


\hline
MPI  \break \cite{jiang2023evaluating}& Self-assessment, Exhibition & built upon International Personality Item Pool (IPIP) with IPIP-NEO and BFI-S& \href{https://github.com/jianggy/MPI/tree/main/inventories}{https://github.com/jianggy/MPI/tree/\break main/inventories}\\

\hline
PersonaChat \break \cite{safdari2023personality} & Self-assessment, Exhibition &  1,155 fictional human persona descriptions & \href{https://github.com/google-research/google-research/tree/master/psyborgs/datasets}{https://github.com/google-research/google-research/tree/master/psyborgs/datasets}\\


\hline
\cite{stockli2024personification} & Self-assessment,Exhibition &the 120 questions on the Big Five Test &\href{ https://bigfive-test.com/test}{ https://bigfive-test.com/test}\\

\hline
\cite{stockli2024personification} & Self-assessment,Exhibition &MBTI test&\href{  https://www.truity.com/test/type-finder-personality-test-new }{ https://www.truity.com/test/
type-finder-personality-test-new }\\
\hline
\cite{huang2023chatgptMBTI} & Self-assessment, Exhibition & MBTI personality tests in different language environments, emotional context induction, and specific persona role-playing & \href{https://github.com/CUHK-ARISE/LLMPersonality/tree/main/dataset}{https://github.com/CUHK-ARISE/LLMPersonality/tree/main/dataset} \\

\hline
\cite{pan2023llms} & Self-assessment, Exhibition & 93 multiple-choice questions to explore MBTI& \href{https://github.com/HarderThenHarder/transformers_tasks/tree/main/LLM/llms_mbti}{https://github.com/HarderThenHarder/\break transformers\_tasks/tree/main/LLM/\break llms\_mbti} \\
% \bottomrule

%MPI的人类结果
%IPIP120 & The dataset measuring thirty facets of the five-factor model with a 120-item public domain inventory. & \href{https://osf.io/tbmh5/}{Johnson's IPIP-NEO data repository} / 
%        \cite{JOHNSON201478}. & \cite{jiang2023evaluating} \\

%Bidimensional Impression Management Index & The dataset contains 20 Likert-type items measuring agentic management and communal management as forms of impression management or socially desirable responding as a faking 10 strategies.& \cite{blasberg2014bidimensional} & \cite{bodroza2023personality} \\

%Self-Consciousness Scales–Revised(SCS-R) & It contains 22 Likert-type items measuring private self-consciousness, public self-consciousness, and social anxiety. & \cite{scheier1985self} & \cite{bodroza2023personality} \\


% \bottomrule
\hline
\end{tabular}
\end{center}
\caption{Overview of Existing Studies}
\label{likert_scales}
\end{table*}



\begin{table*}[h]
\centering
\tiny
\renewcommand{\arraystretch}{1.2}
\begin{center}
\begin{tabular}{p{3cm}m{3cm}m{4cm}m{4cm}}
\hline
\textbf{Dataset} & \textbf{Personality Model} & \textbf{Descriptions} & \textbf{Download Links} \\
\hline
Situational Evaluation of Social Intelligence \break \cite{xu2024academically}& Big-five & 100 corresponding questions as test items for each sub-capacity of social intelligence & \href{https://github.com/RossiXu/social_intelligence_of_llms/}{https://github.com/RossiXu/social\_intelligence\_of\_llms} \\

PHAnToM \break \cite{tan2024phantom}& Big-five, Dark Triad & FANTOM dataset and the ToM task dataset provided in theory-of-mind reasoning tasks & \href{https://anonymous.4open.science/r/PHAnToM/}{https://anonymous.4open.science/\break r/PHAnToM/} \\

Anthropic's Persona \break \cite{choi2024picle}& Big-five(Only A, C and N), Dark Triad and others & The dataset contained 99 different personality types, each with 500 statements that matched and 500 statements that did not match that personality trait. The dataset was randomly divided into 700 training samples and 300 test samples. & \href{https://huggingface.co/datasets/Anthropic/model-written-evals}{https://huggingface.co/datasets/Anthropic/\break model-written-evals}\\

PersonalityEdit \break \cite{mao2024editing}& Big-five (Only A,E, and N) & based on the theory of Social Psychology by generating responses that align with specific topics and targeted personality traits using GPT4& \href{https://github.com/zjunlp/EasyEdit}{https://github.com/zjunlp/EasyEdit} \\


PersonaLLM  \break \cite{jiang2023personallm}& Big-five & BFI personality test, Essays dataset, Reddit Relationships community posts, and story evaluation data from the Prolific platform & \href{https://github.com/hjian42/PersonaLLM}{https://github.com/hjian42/PersonaLLM} \\

Behavior and Self-awareness \break  \cite{cui2023machine}& MBTI & Behaviour dataset is the meticulously processed Alpaca dataset to create a dataset tailored for fine-tuning LLMs. Self-awareness datasets are generated ChatGPT guided by certain prompts.& \href{https://github.com/PKU-YuanGroup/Machine-Mindset/tree/main/datasets}{https://github.com/PKU-YuanGroup/Machine-Mindset/tree/main/datasets} \\

\cite{lacava2024open} & MBTI & 93 multiple-choice questions to explore MBTI & \href{https://www.16personalities.com/}{https://www.16personalities.com/}\\

\cite{petrov2024limited} & Big-five, Others &First is 150 generic persona descriptions randomly sampled from the PersonaChat dataset. Second is 1,000 silicon personas based on the BBC personality dataset.&\href{https://github.com/nikbpetrov/simulation-examples}{https://github.com/nikbpetrov/simulation-examples}\\

\cite{wang2024incharacter} & MBTI &  Datasets sourced from the ChatHaruhi and RoleLLM projects, encompassing 32 widely recognized characters primarily from popular fictional works & \href{https://github.com/Neph0s/InCharacter/tree/main/data}{https://github.com/Neph0s/InCharacter\break /tree/main/data} \\

\cite{huang2023revisiting}& Big-five & BFI comprises 44 items, each rated on a five-point Likert scale.  & \href{https://github.com/CUHK-ARISE/LLMPersonality/tree/main/dataset}{https://github.com/CUHK-ARISE/LLMPersonality/tree/main/dataset} \\

\cite{klinkert2024driving}& Big-five & A cleaned Big Five personality test dataset & \href{https://gitlab.com/humin-game-lab/artificial-psychosocialframework/-/tree/master/LLM\%20Personality}{https://gitlab.com/humin-game-lab/artificial-psychosocialframework/-/tree/master/LLM\%20Personality}\\

\cite{frisch2024llm} & Big-five & BFI comprises 44 items, each rated on a five-point Likert scale. & \href{https://github.com/ivarfresh/Interaction_LLMs}{https://github.com/ivarfresh/\break Interaction\_LLMs} \\

\hline
\end{tabular}
\end{center}
\caption{\textcolor{red}{Not checked} Open source datasets for LLM's personality exhibition}
\label{exhibition_resources}
\end{table*}





\begin{table*}[h]
\centering
\tiny
\renewcommand{\arraystretch}{1.2}
\begin{center}
\begin{tabular}{p{3cm}m{3cm}m{4cm}m{4cm}}
\hline
\textbf{Dataset} & \textbf{Personality Model} & \textbf{Descriptions} & \textbf{Download Links} \\
\hline
\cite{rao-etal-2023-chatgpt}   & MBTI &  Questionnaires with 60 questions  &  \href{https://github.com/Kali-Hac/ChatGPT-MBTI}{https://github.com/Kali-Hac/ChatGPT-MBTI}\\

Essays \break \cite{pennebaker1999linguistic} &  Big-five & 2,468 self-report essays from more than 1,200 students & *no official download link\\
PAN & Big-five & 294 users' tweets and their Big-Five personality scores obtained by the BFI-10 questionnaire&\href{https://pan.webis.de/clef15/pan15-web/author-profiling.html}{https://pan.webis.de/clef15/pan15-web/author-profiling.html}\\
Kaggle & MBTI & 8,675 users, with each user contributing 45-50 posts & \href{https://www.kaggle.com/datasets/datasnaek/mbti-type}{https://www.kaggle.com/datasets\break /datasnaek/mbti-type}\\
Pandora & MBTI & Dozens to hundreds of posts from each of the 9,067 Reddit users & \href{https://psy.takelab.fer.hr/datasets/all/}{https://psy.takelab.fer.hr/datasets/all/} \\
FriendsPersona & Big-five & 711 short conversations are extracted and annotated from the first four seasons of Friends TV Show transcripts &\href{https://github.com/emorynlp/personality-detection}{https://github.com/emorynlp/personality-detection} \\
CPED & Big-five & 12K dialogues in multi-modal context from 40+ TV shows&\href{https://github.com/scutcyr/CPED}{https://github.com/scutcyr/CPED}\\
First Impression & Big-five & 10,000 Youtube video clips of people facing and speaking & \href{https://chalearnlap.cvc.uab.cat/dataset/24/description/}{https://chalearnlap.cvc.uab.cat/dataset/24/description/}\\

\cite{peters2024large} &Big-five & Dialogues of 566 participants with a chatbot built on the ChatGPT &\href{https://osf.io/edn3g/.}{https://osf.io/edn3g/.}\\

\cite{cao2024large} & Big-five &  Demographics of 11,341 public figures from Pantheon 1.0 with manually rated personality traits. & \href{https://osf.io/854w2/}{https://osf.io/854w2/}\\
\hline
\end{tabular}
\end{center}
\caption{Open source datasets for LLM's personality recognition}
\label{recognition_resources}
\end{table*}

==> Self-assessment.tex <==
\section{LLM's Personality Self-assessment}
\label{LLM's Personality Self-assessment}

\textit{Does a LLM possess a stable personality trait?} This question arises from the highly coherent and human-like conversational experience provided by LLMs during interactions, which drives researchers to investigate whether LLMs have acquired intrinsic personality traits in pre-training \cite{pellert2022ai}. Some studies \cite{huang2023chatgptMBTI, pan2023llms} suggest that ChatGPT approximates a stable ENFJ personality type in the MBTI model, while others indicate that LLMs do not consistently maintain a personality trait in assessments \cite{pellert2022ai,miotto2022gpt}. The discrepancy may stem from variations in methodology or the inherent adaptability of LLMs to different conversational contexts. Understanding LLMs' personalities not only helps enrich the user experience by fostering engaging and empathetic interactions but also plays a crucial role in uncovering latent biases, mitigating the biases, and thereby enhancing the fairness and accuracy of LLMs \cite{karra2022estimating}. 

\subsection{Problem Definition}
We first define the LLM's Personality Self-assessment problem as: \textbf{How to measure LLMs’ intrinsic personality traits?} This problem is based on two important assumptions: (1) LLMs possess intrinsic personalities: LLMs have acquired intrinsic personalities from pre-training data (2) LLMs' personalities are measurable: psychometric methods designed for analyzing the personalities of humans are also suitable for LLMs.

When assessing human personality, researchers commonly employ personality questionnaires and self-report essays. Similarly, existing studies also conduct two main approaches to investigate the intrinsic personality traits of LLMs:  (1) prompting LLMs with Likert scale personality questionnaires, and (2) analyzing the textual responses of LLMs. We will introduce these methods in the following content.

\subsection{Likert scale questionnaires}

Likert scale-based personality questionnaires (\textit{e.g.}, Table \ref{BFI_example}) consist of a series of multiple-choice questions (MCQs) that translate respondents' selections into numeric scores, which are then aggregated to produce a final result. These instruments are commonly used in the social sciences to assess human personality traits. Although MCQs are quite natural for humans, LLMs are designed for open-ended text input and output, making it difficult for them to conduct MCQs directly. Therefore, researchers have tried various methods to input the questionnaires to LLMs and then analyze their text responses to derive the personality assessment results.

Most studies prompt LLMs directly with questionnaire questions and options \cite{song2023large,safdari2023personality,frisch2024llm}. However, these methods require additional approaches, such as utilizing regular expressions \cite{jiang2023evaluating}, designing text parsers \cite{li2023does}, or analyzing the probability values of the last token in the text response \cite{pan2023llms} to extract the answer options from the LLMs' text responses. Faced with this issue, some studies \cite{lacava2024open,stockli2024personification} found that adding instructive task descriptions and constraints besides the questions in prompts, such as \textit{You will be provided a question ... to test your personality}, can facilitate obtaining questionnaire answers from LLMs.

Besides, since most LLMs, such as ChatGPT and Llama-chat, are configured to decline queries about personal opinions and experiences, this poses challenges for LLMs responding to personality questionnaires. To address this issue, some researchers attempted to instruct LLMs to respond with only a number within the Likert scale levels \cite{huang2023chatgpt}, rephrase the items in the questionnaire into the third person plural \cite{miotto2022gpt3} or add the role description \cite{sorokovikova2024llms} to eliminate this constraint.

In addition to the common generative LLMs, some researchers also assessed the personalities of earlier pre-trained large language models by reformulating questions in questionnaires into various Natural Language Understanding (NLU) tasks. For instance, \citet{caron2022identifying} modifies the questionnaire by incorporating blanks within questions and then prompts BERT to fill the answer options into the masked positions.  \cite{pellert2022ai} utilized natural language inference (NLI) techniques to enable models such as DeBERTa to identify the most appropriate options corresponding to the questions in the questionnaires.

% 用量表的大多都考虑温度，重复多次实验

\begin{table}[t]
    \centering
    \linespread{1}
    \renewcommand{\arraystretch}{1.3}
    \begin{tabular}{p{7cm}}
 	\toprule
 	\textit{I see myself as someone who is helpful and unselfish with others.}   \\
	\hline
	\textit{1 = Disagree strongly} \\
	\textit{2 = Disagree a little} \\
	\textit{3 = Neither agree nor disagree} \\
	\textit{4 = Agree a little} \\
	\textit{5 = Agree strongly} \\
	\hline
	\textit{Please write a number to indicate the extent to which you agree or disagree with that statement.}\\
	\bottomrule
    \end{tabular}
    \caption{The 7-th question in the BFI \cite{john1999big}.}
    \label{BFI_example}
\end{table}



\subsection{Text response analysis}

Despite most existing studies utilizing questionnaires to assess the personalities of LLMs, some researchers \cite{dorner2023personality, huang2023revisiting} question whether LLMs, which are primarily designed for generating text content, can produce meaningful options when answering multiple-choice questions in questionnaires. Consequently, there are also studies that perform text analysis from semantic or linguistic perspectives on the responses of LLMs to determine their personalities.

\cite{karra2022estimating} classifies the text responses of LLMs to a personality questionnaire into the big five personality traits using a Zero-shot classifier. Similarly, \cite{pellert2022ai} prompted the questions from personality inventories recorded the language models' responses, and conducted zero-shot classification to obtain their personality scores. While \cite{hilliard2024eliciting} measures the Big Five personality traits of LLMs by further classify their responses to prompts derived from standard interview questions with fine-tuned text classifiers. Besides end-to-end text classifiers, Linguistic Inquiry and Word Count (LIWC, \citet{pennebaker2001linguistic}), a text analysis tool for personality recognition is also adopted in existing studies \cite{frisch2024llm,gu2023effectiveness,jiang2023personallm} for personality assessment of LLMs. It's worth mentioning that \cite{jiang2023evaluating} also conducts the vignette test \cite{kwantes2016assessing} to assess the personality exhibited by LLMs. They prompt LLMs with the context that describes a real-world scenario, followed by an open question and instructions for a short essay. Then, human participants were recruited to assess the generated responses of LLMs in personality reflection.

\subsection{Assessment Results Analysis}

Based on the various assessment methods introduced above, researchers have obtained the results of personality of LLMs. In general,  although the results are similar in some aspects (\textcolor{red}{citation}), they are different as a whole. These differences depend on a variety of factors: measurement approaches, model versions, hyperparameters, and so on. However, extensive results \cite{li2023does,huang2023chatgpt} agree on the worrisome tendencies to score high on the Dark Triad of narcissism, psychopathy, and Machiavellianism, demanding more rigorous research on the safety of these models.

Due to the diversity of the assessment results, researchers investigate the robustness of the assessments from different aspects. Although multiple terms are used and interpreted, such as reliability \cite{huang2023revisiting}, stability \cite{shu2024dont}, self-consistency \cite{pellert2022ai}, and validity \cite{romero2023gpt}, we summarize these terms mainly are from two perspectives:
\textbf{Reliability}, which refers to measurement precision and can be approximated by the consistency of answers and the stability of test results over multiple repetitions; and \textbf{Validity}, which refers to the extent to which a test measures what it claims to measure, in other words, whether the personality assessment approaches used are indeed applicable to measuring the personalities of LLMs \cite{dorner2023personality}. The former explores the results from the perspective of the LLMs, while the latter investigates from the perspective of the assessment approaches.

\subsubsection{Reliability}
Several studies have reported achieving high reliability in the personality assessments of LLMs. \cite{huang2023revisiting} conducted a comprehensive analysis of responses across 2,500 experimental conditions, demonstrating that GPT-3.5-turbo exhibits consistent behavior in responses to the Big Five Inventory. \cite{jiang2023evaluating} further bolstered this notion, performing multiple analyses to illustrate that GPT-3.5 can manifest consistent personality tendencies throughout numerous evaluations. In a related study, \cite{huang2023chatgptMBTI} showcased that ChatGPT consistently exhibits the ENFJ personality type across diverse languages, prompts, question orders, and rephrased inquiries in assessments.

However, not all findings are in agreement. \cite{li2023does}, while asserting that GPT-3 displays relatively consistent personality traits, also identified instances of conflicting answers and discrepancies in the responses generated by LLMs attributable to variations in the order of options within prompts. \cite{gupta2024selfassessment} discovered that the test scores of ChatGPT and Llama-2 are not consistently robust across equivalent prompts and differing option presentations. Additionally, \cite{miotto2022gpt3} reported that GPT-3’s personality profile fluctuates with the adjustment of temperature values in the model's settings. \cite{song2023large} observed \textcolor{red}{inherent biases} within LLMs, leading to a tendency to produce identical answers irrespective of the situational context being tested.

Building upon these insights, \cite{serapiogarcía2023personality} has underscored the significance of testing various model versions and sizes, employing a larger parameter volume, and leveraging Supervised Fine-Tuning techniques to augment the reliability of personality assessments in LLMs.

\subsubsection{Validity}

The discussion on the validity of personality assessments for LLMs is also not marked by a consensus. \cite{jiang2023evaluating} incorporated a validity assessment by prompting LLMs to explain the reason for selecting particular options within Likert-scale personality questionnaires. The responses successfully indicated that LLMs displayed a strong understanding of the question items, highlighting their research validity. Nonetheless, upon conducting an exhaustive analysis of the responses from LLMs to personality questionnaires, researchers failed to discern patterns that were both intended in the design and observed in human subject pools \cite{dorner2023personality}. In conclusion, before conducting personality assessments for LLMs, validity cannot be assumed without a thorough and critical analysis.

\subsection{Findings and Open Challenges}
\subsubsection{Findings}
We summarize the findings derived from existing studies by answering the following questions: \\

\noindent
\textbf{1. How do people assess the personalities of LLMs?} Although some studies use semantic analysis or linguistic tools to infer the personality of LLMs from their text responses, most work still relies on prompt engineering to instruct LLMs to complete questionnaires to reveal their inherent personality traits. \\

\noindent
\textbf{2. What are the assessment results?}
Results obtained from different studies show significant variability, with no consensus on LLM personality traits due to diverse methodologies and a lack of standardized benchmarks. However, some studies agree that LLMs often exhibit darker traits than humans, likely due to the varied training data they are exposed to. \\

\noindent
\textbf{3. Are the assessments meaningful?}
Although most existing work considers multiple repetitions, prompt wording, and the order of questions and options in the questionnaire to obtain more reliable measurements, the validity of using questionnaires or text analysis to measure LLM personality from a psychometric perspective has not yet been verified. A thorough and critical analysis of the assessment approach is essential for obtaining meaningful results.

\subsubsection{Open Challenges}

\noindent
\textbf{Absence of Assessment Benchmarks}: The results of LLMs' personality self-assessments have shown significant variability. This inconsistency arises from diverse methodologies, prompting styles, and evaluation criteria used in different studies. A standardized benchmark unifying the assessment methods can contribute to comparable and more meaningful results. \\

\noindent
\textbf{Dark traits elimination in LLMs}: LLMs are uncovered to often exhibit traits that are considered darker or more negative compared to the average human personality. This may cause misinformation, loss of trust, ethical concerns, and potential harm to users' mental health. Effectively eliminating these traits while retaining the excellent interactive capabilities of LLMs remains an open question.

==> preliminary.tex <==
\section{Overview}

In this section, we present a comprehensive overview of existing studies based on statistical results on our categorization. We have collated a total of 60 released scientific papers from publicly available corpora in LLM's understanding of personality since 2022, encompassing investigations, methodologies, and applications. 

The number of papers in this emerging domain has been increasing annually, and even as of June 2024, the volume of publications released has already surpassed that of the entire previous year. This indicates a growing popularity and interest in the field, as shown in Figure \ref{fig: trends}. Concurrently, we observe a substantial body of work on LLMs' personality self-assessment, reflecting a sustained interest in exploring the intrinsic characteristics of LLMs. Following closely is research on LLMs' personality exhibition, which underscores the increasing focus on LLM-based interactions in various scenarios. 
Compared to the two new research problems, there is relatively less work on LLMs in personality recognition. This may be attributed to the fact that personality recognition, as a classical text classification problem, has been already widely studied with traditional methods. Nevertheless, personality recognition based on LLMs remains crucial in LLM-based interactions. The number of studies on this topic also continues to grow annually.

\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{emnlp2024/figs/Trends_in_LLM_Personality.pdf}
    \caption{Trends in LLM Personality Research}
    \label{fig: trends}
\end{figure}





\subsection{Personality Models}
In reviewed literature, researchers commonly adopt personality models based on the trait theory \textcolor{red}{citation}, where the personalities of individuals are defined as several aspects of stable and consistent patterns of behavior, emotion, and cognition, as shown in Figure \ref{fig: personality models}. 

The most commonly adopted personality model among the existing three research problems is the Big-five model \cite{de2000big}, which includes five core dimensions: openness, conscientiousness, extraversion, agreeableness, and neuroticism. These dimensions capture various aspects of an individual's personality, ranging from their inclination towards new experiences to their level of emotional stability. Another widely recognized personality assessment model is the Myers-Briggs Type Indicator (\textbf{MBTI}) \cite{Myers_1962}, which categorizes individuals into one of 16 personality types based on their preferences in four dichotomous dimensions: extraversion/introversion, sensing/intuition, thinking/feeling, and judging/perceiving. 

Besides the comprehensive personality models, researchers are also interested in the potential dark personality traits of LLMs, such as the Short Dark Triad-3 (SD-3, \citet{jones2014introducing}), or Dark Triad Dirty Dozen (DTDD, \citet{jonason2010dirty})  which measures Machiavellianism (a manipulative attitude), narcissism (excessive self-love), and psychopathy (lack of empathy), capturing the darker aspects of human nature.

In addition to the aforementioned personality models, researchers are also interested in (1) their variant models, such as the Eysenck Personality Questionnaire-Revised (EPQ-R) \cite{eysenck1985revised} assessing the dimensions of extraversion, neuroticism, and psychoticism, or the HEXACO model \cite{ashton2009hexaco} measuring honesty-humility in addition to the Big-five traits;  or (2) other psychological aspects in LLMs, such as motivations or interpersonal relationships \cite{huang2023chatgpt,bodroza2023personality}.




\begin{figure}[t]
    \centering
    \includegraphics[scale=0.32]{emnlp2024/figs/personality_model_in_llm_research.pdf}
    \caption{Personality Model in LLM}
    \label{fig: personality models}
\end{figure}


\subsection{Large Language Models}

In existing studies, there is a significant interest in the performance of various LLMs on the three research problems, as shown in Figure \ref{fig: llms}. Among all the LLMs, the GPT series models have garnered the most attention from researchers. Though most of them are not directly open-sourced, extensive researchers (\textit{e.g.}, \textcolor{red}{citation}) have explored their performance in personality understanding through API. Additionally, several well-known open-source LLMs, such as the Llama series \textcolor{red}{citation}, Mixtral \textcolor{red}{citation}, and Falcon \textcolor{red}{citation}, have also attracted a lot of attention.

Among all LLMs, the task that researchers have focused on the most is personality self-assessment. Despite LLMs typically referring to models after the occurrence of GPT-3, we also found that some pioneering work has already attempted to measure potential personality traits exhibited by BERT and GPT-2 \textcolor{red}{citation}.






 \begin{figure*}[t]
     \centering
     \includegraphics[scale=0.4]{emnlp2024/figs/model_in_llm_research.pdf}
     \caption{Enter Caption}
     \label{fig:llms}
 \end{figure*}






% One prominent framework for understanding personality is the Big Five model \cite{de2000big}, which includes five core dimensions: openness, conscientiousness, extraversion, agreeableness, and neuroticism. These dimensions capture various aspects of an individual's personality, ranging from their inclination towards new experiences to their level of emotional stability. Another widely recognized personality assessment tool is the Myers-Briggs Type Indicator (MBTI) \cite{Myers_1962}, which categorizes individuals into one of 16 personality types based on their preferences in four dichotomous dimensions: extraversion/introversion, sensing/intuition, thinking/feeling, and judging/perceiving. Based on the above models, the Eysenck Personality Questionnaire \cite{eysenck1985revised} is also proposed for assessing the dimensions of extraversion, neuroticism, and psychoticism in personality traits. 

% \subsection{Personality Assessment}

% \begin{itemize}
% \item \textbf{Big Five Inventory (BFI):} The Big Five personality traits, namely, extraversion (emotional expressiveness), agreeableness (trust and kindness), conscientiousness (thoughtfulness), neuroticism (emotional instability), and openness (openness to experience), are the most widely accepted and commonly used personality models in academic psychology. BFI \cite{john1999big} consists of 44 statements that must be rated from 1 to 5 based on how much the respondent agrees with them.

% \item \textbf{HEXACO:} Personality was measured via the 60-item Hexaco questionnaire \cite{ashton2009hexaco}. The Hexaco is a 6-dimensional model of personality, measuring the facets of honesty-humility, emotionality, extraversion, agreeableness, conscientiousness, and openness to experience.

% \item \textbf{Short Dark Triad-3:} The dark triad personality consists of three closely related but independent personality traits that have a malevolent connotation \cite{jones2014introducing}. The three traits, namely, Machiavellianism (a manipulative attitude), narcissism (excessive self-love), and psychopathy (lack of empathy), capture the dark aspects of human nature. These three traits share a common core of callous manipulation and are strong predictors of a range of antisocial behaviors, including bullying, cheating, and criminal behaviors (Furnham et al., 2013). SD-3 is a uniform assessment tool for the three traits. This test consists of 27 statements that must be rated from 1 to 5 based on how much the respondent agrees with them. The scores of statements under a trait are averaged to calculate the final score of the trait.
% \end{itemize}




==> tables.tex <==



--------


\begin{table*}[h]
\centering
\scriptsize
% \linespread{1}
\renewcommand{\arraystretch}{1.2}
% \begin{tabular}{m{4cm}m{4cm}cm{5cm}}
\begin{center}
\begin{tabular}{|p{3cm}|p{4cm}|m{4cm}|m{4cm}|}
% \toprule
\hline
\textbf{Methods} & \textbf{Backbone LLMs} & \textbf{Personality Models} & \textbf{Descriptions} \\


\hline
\cite{karra2022estimating} & GPT-2,3,3.5-turbo; \textcolor{red}{LLama}; Transformer-XL; XLNet & Big-five & Personality assessment of LLMs\\
\cite{bodroza2023personality} & GPT-3 (text-davinci-003) & Big-five, HEXACO, Dark Triad, and other psychological aspects & Self-assessment through psychological questionnaires \\
\cite{miotto2022gpt} & GPT-3 & HEXACO & Personality assessment of LLMs\\
\cite{li2023does} & GPT-3,3.5,4; InstructGPT; Llama2-chat-7B & Big-five, Dark Traid & Evaluating psychological safety of LLMs\\
\cite{huang2023revisiting} & GPT-3.5-turbo &Big-five & Self-assessment \\
\cite{huang2023chatgpt} & text-davinci-003; GPT-3.5-turbo,4; Llama-2-7B,13b & Big-five; EPQ-R; Short Dark Triad, and other psychological aspects & Self-assessment\\
\cite{wang2024incharacter} & GPT-3.5,4; Gemini & Big-five, MBTI & Personality assessment of role-playing agents\\
\cite{romero2023gpt} & GPT-3 & Big-five &  Personality assessment of LLMs \\


\cite{hilliard2024eliciting} & GPT-2,3.5,4 (all series); Llama-2 (all series); Mixtral-7B (all series); Felcon-7B,7B-Instruct; Bloom(z)-(all series); OPT-125M,350M,1.3B & Big-five & Self-assessment by text classification \\
\cite{pellert2023ai} & multilingualDeBERTa; DistilRoBERTa; BART; XLMRoBERTa; DeBERTa; DistilBART & Big-five; Value Orientations; Moral Norms; Beliefs About Gender & Self-assessment \\
\cite{caron2022identifying} & BERT-base; GPT-2 & Big-five & Self-assessment by questionnaires \\

\cite{song2023large} & GPT2-XL-1.5B;GPT-Neo-2.7B;GPT-NeoX-20B;OPT-13B,30B & Big-five & Self-assessment \\
\cite{dorner2023personality} & Llama-2-chat-70B; GPT-3.5,4 & Big-five & Self-assessment\\
\cite{sorokovikova2024llms} & GPT-4; Llama-2-70B-chat; Mistral-8x-7B; & Big-five & Self-assessment \\
\cite{shu2024dont} & GPT-2,3.5,4; Falcon-7B; BLOOMZ (all series); Llama2-7B,7B-chat,13B,13B-chat; RedPajama-7B; and FLAN-T5 (all series) & MODEL-PERSONAS (Proposed in this work) & Assessing the reliability of self-assessment\\
\cite{gupta2024selfassessment} & ChatGPT; Llama2-7B, 13B, 70B & Big-five & Evaluating Robustness of Self-assessment\\

\textcolor{red}{\cite{lacava2024open}} & Mixtral-7B,-8x-7B; Llama2-7B-chat,-13B; SOLAR-10.7B; Neural-Chat-7B; Dolphin-2.1; Vicuna-7B; Falcon-7B; Phi-2 & MBTI & \textcolor{red}{Aware}, Self-assessment, Exhibition, mimicking specific roles\\

\cite{pan2023llms} &ChatGPT; GPT-4; Bloom-7B; Baichuan-7B,13B; OpenLlama-7B-v2 & MBTI& Self-assessment; Exhibition \\
\cite{jiang2023evaluating} & GPT-3.5 & Big-five & Self-assessment, Exhibition\\
\cite{safdari2023personality} &PaLM-62B; Flan-PaLM-8B,62B,540B; Flan-PaLMChilla-62B & Big-five & Self-assessment, Exhibition\\


%%%下面是新的





\cite{ai2024cognition} & ChatGLM3,GPT-3.5-turbo,GPT-4,Vicuna-13b,Vicuna-33b & Big-five,MBTI & Self-assessment\\

\cite{song2024identifying} & ChatGPT, Llama2 & MBTI & Self-assessment\\

\cite{salecha2024large} & OpenAI’s text-davinci-002, GPT-3.5, and GPT-4, Anthropic’s Claude 3
Opus, Claude 3 Haiku, Google’s PaLM 2,
and Meta’s Llama 3 70B Instruct, Llama 2 70B Chat.& Big-five & Self-assessment\\

\cite{kovavcevic2024personality} & GPT-3 &Big-five, Others & Others\\

\cite{stockli2024personification} &GPT4&Big-five,MBTI& Self-assesment,Exhibition\\

\cite{barua2024psychology}&GPT4,GPT3,FLAN-T5-XXL&Dark Triad,Big-five & Self-assesment\\

\cite{yu2023personality}& ChatGPT, BARD & Big-five & Self-assessment\\

\cite{huang2023chatgptMBTI} & text-davinci-003, ChatGPT, GPT-4; Bard, Spark, ERNIE Bot, ChatGLM & MBTI & \textcolor{red}{Self-assessment} (multi-lingual), Exhibition\\

% \bottomrule
\hline
\end{tabular}
\end{center}

\caption{Overview of Existing Studies Self-assessment}
\label{likert_scales}
\end{table*}







\begin{table*}[h]
\centering
\scriptsize
% \linespread{1}
\renewcommand{\arraystretch}{1.2}
% \begin{tabular}{m{4cm}m{4cm}cm{5cm}}
\begin{center}
\begin{tabular}{|p{3cm}|p{4cm}|m{4cm}|m{4cm}|}
% \toprule
\hline
\textbf{Methods} & \textbf{Backbone LLMs} & \textbf{Personality Models} & \textbf{Descriptions} \\

\hline
*\cite{xu2024academically} &GPT(all series); Vicuna-13B,33B; Llama-2-chat(all series); Mixtral-7B,8x7B &Big-five & Probing the influence of Personality Exhibition\\

\cite{karra2022estimating} & GPT-2,3,3.5-turbo; \textcolor{red}{LLama}; Transformer-XL; XLNet & Big-five & Exhibition\\

\cite{safdari2023personality} &PaLM-62B; Flan-PaLM-8B,62B,540B; Flan-PaLMChilla-62B & Big-five & Self-assessment, Exhibition\\

\cite{stockli2024personification} &GPT4&Big-five,MBTI& Self-assesment,Exhibition\\

\textcolor{red}{\cite{lacava2024open}} & Mixtral-7B,-8x-7B; Llama2-7B-chat,-13B; SOLAR-10.7B; Neural-Chat-7B; Dolphin-2.1; Vicuna-7B; Falcon-7B; Phi-2 & MBTI & \textcolor{red}{Aware}, Self-assessment, Exhibition, mimicking specific roles\\

\cite{jiang2023evaluating} & GPT-3.5 & Big-five & Self-assessment, Exhibition\\

\cite{pan2023llms} &ChatGPT; GPT-4; Bloom-7B; Baichuan-7B,13B; OpenLlama-7B-v2 & MBTI& Self-assessment; Exhibition \\
*\cite{tan2024phantom} & GPT-3.5; Llama2-\textcolor{red}{7B}; Mistral-7B; Falcon-7B; Zephyr-7B-Beta & Big-five, Dark Triad & Investigating effects of inducing personality on reasoning\\
\cite{jiang2023personallm} & GPT-3.5,4 & Big-five& Make LLM to express personality\\
*\cite{li2024tailoring} & Llama2-7B-chat; OpenChat3.5-7B; Neural-chat-7B; Baichuan2-7B-Chat; Llama2-13B-chat & Big-five & Tailoring Personality Traits in LLMs \\
\cite{li2023does} & GPT-3,3.5,4; InstructGPT; Llama2-chat-7B & Big-five, Dark Traid & Evaluating psychological safety of LLMs\\
\cite{ramirez2023controlling} & Jurassic-1-Jumbo-175B & Big-five & Exhibition \\
\cite{noever2023ai} & ChatGPT & Big-five & Exhibition \\
\cite{cui2023machine} & ChatGPT & MBTI & Exhibition (Proposed a dataset and a training procedure) \\
\cite{mao2024editing} & GPT-J-6B & Big-five (Only A,E, and N) & Exhibition \\
\cite{huang2023chatgptMBTI} & text-davinci-003, ChatGPT, GPT-4; Bard, Spark, ERNIE Bot, ChatGLM & MBTI & \textcolor{red}{Self-assessment} (multi-lingual), Exhibition\\


%下面是新的
\cite{noh2024llms}  & gpt-4-turbo & Big-five & Exhibition,different personality agents to negotiate with each other\\

\cite{phillips2024can}  & ChatGPT-3.5, ChatGPT-4, Jasper, and Google Bard & Big-five & Exhibition,Faking on personality tests \\

\cite{klinkert2024driving}  & text-davinci-003,gpt-3.5-turbo-0613,gpt-4-0613 & Big-five & Exhibition,Generative Agents With Their Personality \\

\cite{liu2024dynamic}  & GPT-4, GPT-3.5, Glm3-3B-Chat, Yi-6B-Chat, Llama2-7B-Chat-hf & Big-five & Exhibition, \textcolor{red}{Personality Recognition}\\
%这里的性格辨别是自动从对话中评估人物的性格特征

\cite{weng2024controllm}  & Llama-2-Chat 7B,Llama-2-Chat 70B,Falcon-7B & Big-five & Exhibition\\

\cite{kovac2023large}  & GPT-3.5-turbo-0301,GPT-4-0314,Davinci-003,Upstage-LLaMa-65B-instruct,Upstage-LLaMa-2-70B-instruct,Redpajama-incite-7b-chat,Redpajama-incite-7b-instruct,StableLM,StableVicuna,Zephyr-7b-beta & Big-five & Exhibition, decision-making abilities of LLMs post role-playing\\

\cite{shen2024decisionmaking}  & ChatGPT & MBTI, Dark Triad & Exhibition, guide the model in eliciting a specific target persona\\

\cite{choi2024picle}  & llama-2-7b-chat-hf, vicuna-7b-v1.5, gpt-j-6b  & Big-five(Only A,C and N),Dark Traid and others & Exhibition\\
%%%%少写了dark traid！！！！！




\cite{gu2023effectiveness}  & gpt3.5, gpt4  & optimistic/pessimistic & Exhibition,persistent conversational agent personalities\\


%新的
\cite{he2024afspp}  & gpt4  & MBTI, Dark Triad & Exhibition,social networks and identity shape personalities \\

\cite{sreedhar2024simulating}  & gpt3.5,gpt4  &  greedy and fair & Exhibition,Human Strategic Behavior\\

\cite{meguellati2024good} & gpt3.5,gpt4  &  Big-five(openness and neuroticism) & generating personalized online advertisements (ads) tailored to specific personality traits\\ %%application

\cite{petrov2024limited}& gpt3.5,gpt4  &  Big-five, Others  & Exhibition, Simulating human psychological behaviours\\

\cite{kaszyca2023possible}& ChatGPT &  Big-five, Others  & Exhibition, mimicking human annotator\\

\cite{de2024use}& ChatGPT &  Big-five,Dark Traid, Others  & Exhibition\\

\cite{liu2024personalityaware}& Zephyr-7B-beta, Vicuna-13B-v1.5, GPT-3.5, GPT-4 &  Big-five  & Exhibition, Conversational Intelligent Tutoring Systems\\

\cite{phillips4826678hacking} 2024 & ChatGPT-3.5, ChatGPT-4, LLaMa2, and Jasper & Conscientiousness and Integrity & Exhibition\\

\textcolor{red}{???}\cite{frisch2024llm} & GPT-3.5-turbo & Big-five & Personality assessment for persona-conditioned LLMs,\textcolor{red}{Exhibition} \\
% \bottomrule
\hline
\end{tabular}
\end{center}

\caption{Overview of Existing Studies Exhibition}
\label{likert_scales}
\end{table*}







\begin{table*}[h]
\centering
\scriptsize
% \linespread{1}
\renewcommand{\arraystretch}{1.2}
% \begin{tabular}{m{4cm}m{4cm}cm{5cm}}
\begin{center}
\begin{tabular}{|p{3cm}|p{4cm}|m{4cm}|m{4cm}|}
% \toprule
\hline
\textbf{Methods} & \textbf{Backbone LLMs} & \textbf{Personality Models} & \textbf{Descriptions} \\


\hline
\cite{rao-etal-2023-chatgpt} & ChatGPT, GPT-4, InstructGPT & MBTI &  Assessing personality recognition ability\\
\cite{hu2024llmvssmall} & GPT-3.5-turbo & MBTI & Personality Recognition\\
\cite{yang2023psycot} & GPT-3.5-turbo & Big-five; MBTI & Personality Recognition \\
\cite{10463124} &GPT-3.5,4 & HEXACO &  Personality Recognition from Asynchronous Video Interviews\\

\cite{wen2024affective} &Llama-2-7B & Big-five & Personality Recognition\\%2024
\cite{ji2023chatgpt} & ChatGPT & Big-five & Personality Recognition\\%2023
\cite{ganesan2023systematic} & GPT-3 & Big-five & Personality Recognition \\%2023
\cite{peters2023large} & GPT-3.5,4 & Big-five & Personality Recognition\\%2023

\cite{peters2024large} & GPT-4 & Big-five & Personality Recognition\\



\cite{derner2023chatgpt} & ChatGPT & Big-five & Personality Recognition\\

\cite{amin2023chatgpts} & RoBERTa, ChatGPT & Big-five,Others & Personality Recognition\\

\cite{cao2024large}& GPT-3 & Big-five & Personality Recognition\\

\cite{yu4671511gpt} 2023& ChatGPT & Big-five & Personality Recognition\\

% \cite{liu2024dynamic}  & GPT-4, GPT-3.5, Glm3-3B-Chat, Yi-6B-Chat, Llama2-7B-Chat-hf & Big-five & Exhibition, Personality Recognition\\

 
% \bottomrule
\hline
\end{tabular}
\end{center}
\caption{Overview of Existing Studies recognition}
\label{likert_scales}
\end{table*}

